Sinan: Data-Driven, QoS-Aware Cluster Management for Microservices

Cloud applications are increasingly shifting from large monolithic services, to large numbers of loosely-coupled, specialized microservices. Despite their advantages in terms of facilitating development, deployment, modularity, and isolation, microservices complicate resource management, as dependencies between them introduce backpressure effects and cascading QoS violations. We present Sinan, a data-driven cluster manager for interactive cloud microservices that is online and QoS-aware. Sinan leverages a set of scalable and validated machine learning models to determine the performance impact of dependencies between microservices, and allocate appropriate resources per tier in a way that preserves the end-to-end tail latency target. We evaluate Sinan both on dedicated local clusters and large-scale deployments on Google Compute Engine (GCE) across representative end-to-end applications built with microservices, such as social networks and hotel reservation sites. We show that Sinan always meets QoS, while also maintaining cluster utilization high, in contrast to prior work which leads to unpredictable performance or sacrifices resource efficiency. Furthermore, the techniques in Sinan are explainable, meaning that cloud operators can yield insights from the ML models on how to better deploy and design their applications to reduce unpredictable performance.

==> Implementation.tex <==
\vspace{-0.02in}
\subsection{Sinan Implementation}
\label{sec:implementation}

The data collection is implemented in Python in 6k LoC.
We implement Sinan's centralized scheduler in approximately 3.5k lines of 
Python and 100 lines of C++. The neural network model and boosted tree are 
implemented using MxNet~\cite{mxnet} and XGBoost~\cite{xgboost} with 700 lines of Python. 
The per-node operators are also written in Python in approximately 1,500 lines of Python 
and 100 lines of C++. %{\color{red} does this include everything? data collection, scheduler, per-node agents, etc.? is the distributed operator the per-node agent?} 
%\vspace{-0.02in}
%- if there is space/time, add something about how the scheduler is implemented. Language, LoC, what the ML models are written in, what the per-node monitors do, etc. 

